Generating Aligned Pseudo-Supervision from Non-Aligned Data for Image Restoration in Under-Display Camera

Due to the difficulty in collecting large-scale and perfectly aligned paired training data for Under-Display Camera (UDC) image restoration, previous methods resort to monitor-based image systems or simulation-based methods, sacrificing the realness of the data and introducing domain gaps. In this work, we revisit the classic stereo setup for training data collection -- capturing two images of the same scene with one UDC and one standard camera. The key idea is to "copy" details from a high-quality reference image and "paste" them on the UDC image. While being able to generate real training pairs, this setting is susceptible to spatial misalignment due to perspective and depth of field changes. The problem is further compounded by the large domain discrepancy between the UDC and normal images, which is unique to UDC restoration. In this paper, we mitigate the non-trivial domain discrepancy and spatial misalignment through a novel Transformer-based framework that generates well-aligned yet high-quality target data for the corresponding UDC input. This is made possible through two carefully designed components, namely, the Domain Alignment Module (DAM) and Geometric Alignment Module (GAM), which encourage robust and accurate discovery of correspondence between the UDC and normal views. Extensive experiments show that high-quality and well-aligned pseudo UDC training pairs are beneficial for training a robust restoration network. Code and the dataset are available at https://github.com/jnjaby/AlignFormer.

==> figures/loss_func.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.9\linewidth]{figs/pck_std.pdf}
    \caption{\textbf{PCK on different wrapped images where flows are added with perturbation.}
    }
    \label{fig:pck_std}
\end{figure}

==> figures/ppm.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=.9\linewidth]{figs/seg.pdf}
    \draftfig{0.1}{0.12}{Input}
    \draftfig{0.1}{0.12}{w/o PPM}
    \draftfig{0.1}{0.12}{w/ PPM}

    \caption{\textbf{Ablation study on PPM.}
    }
    \label{fig:ppm}
\end{figure}

==> tables/alignment.tex <==
\begin{table}[t]
\caption{\textbf{Ablation study on alignment method.}
}
 \vspace{-0.3cm}
\label{tab:alignment}
\centering
% \setlength\tabcolsep{2.5pt}
\resizebox{.9\linewidth}{!}{
\begin{tabular}{l|cccc}
\toprule
PCK (\%)$\uparrow$ & Ref & Cai \etal~\cite{cai2019toward} & RAFT~\cite{teed2020raft} & AlignFormer (Ours)
\\\midrule
$\alpha=0.01$ & 18.77 & 20.16 & 52.35 & 55.57  \\
$\alpha=0.03$ & 54.12 & 53.50 & 91.90 & 93.11 \\
$\alpha=0.10$ & 76.52 & 67.47 & 96.75 & 97.47 \\
% \midrule
% PSNR & & \\
% SSIM & & \\
\bottomrule
\end{tabular}
}
 \vspace{-0.5cm}
\end{table}

==> tables/dam.tex <==
\begin{table}[t]
\caption{\textbf{Ablation study on DAM}
}
 \vspace{-0.3cm}
\label{tab:exp_dam}
\centering
% \setlength\tabcolsep{2.5pt}
\resizebox{.6\linewidth}{!}{
\begin{tabular}{l|cc}
\toprule
PCK (\%)$\uparrow$ & w/o DAM & w/ DAM
\\\midrule
$\alpha=0.01$ & 52.47 & 55.57 \\
$\alpha=0.03$ & 91.79 & 93.11 \\
$\alpha=0.10$ & 96.60 & 97.47 \\
% \midrule
% PSNR & & \\
% SSIM & & \\
\bottomrule
\end{tabular}
}
 \vspace{-0.4cm}
\end{table}

==> tables/optical_estimator.tex <==
\begin{table}[t]
\caption{\textbf{Ablation study on optical flow estimator.}
}
\vspace{-0.3cm}
\label{tab:exp_optical}
\centering
% \setlength\tabcolsep{2.5pt}
\resizebox{0.94\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule
Estimator & \blue{Zero} & SpyNet & PWC-Net & RAFT
\\\midrule
PCK@$\alpha=0.01$ & \blue{9.04} & 27.36 & 32.78 & 55.57 \\
PCK@$\alpha=0.03$ & \blue{24.77} & 52.36 & 91.21 & 93.11 \\
PCK@$\alpha=0.10$ & \blue{34.43} & 62.97 & 97.15 & 97.47 \\
\bottomrule
\end{tabular}
}
\vspace{-0.3cm}
\end{table}

==> tables/ppm.tex <==
\begin{table}[t]
\caption{\textbf{Ablation study on PPM.}
}
\label{tab:exp_ppm}
\vspace{-0.3cm}
\centering
% \setlength\tabcolsep{2.5pt}
\resizebox{.7\linewidth}{!}{
\begin{tabular}{c|ccc}
\toprule
 & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
\\\midrule
w/o PPM & 24.29 & 0.8845 & 0.1172 \\
w/ PPM & 24.60 & 0.8855 & 0.1144 \\
\bottomrule
\end{tabular}
}
\vspace{-0.4cm}
\end{table}

==> tables/radius.tex <==
\begin{table}[t]
\caption{\textbf{Ablation study on radius.}
}
\vspace{-0.3cm}
\label{tab:exp_radius}
\centering
% \setlength\tabcolsep{2.5pt}
\resizebox{.7\linewidth}{!}{
\begin{tabular}{c|ccc}
\toprule
Radius & 0 & 1 & 2
\\\midrule
PCK@$\alpha=0.01$ & 53.28 & 55.10 & 55.57 \\
PCK@$\alpha=0.03$ & 92.95 & 93.12 & 93.11 \\
PCK@$\alpha=0.10$ & 97.46 & 97.50 & 97.47 \\
\bottomrule
\end{tabular}
}
\vspace{-0.3cm}
\end{table}
